BLEKeeper: Response Time Behavior Based Man-In-The-Middle Attack Detection

Bluetooth Low Energy (BLE) has become one of the most popular wireless communication protocols and is used in billions of smart devices. Despite several security features, the hardware and software limitations of these devices makes them vulnerable to man-in-the-middle (MITM) attacks. Due to the use of these devices in increasingly diverse and safety-critical applications, the capability to detect MITM attacks has become more critical. To address this challenge, we propose the use of the response time behavior of a BLE device observed in relation to select read and write operations and introduce an activeMITM attack detection system that identifies changes in response time. Our measurements on several BLE devices show that theirresponse time behavior exhibits very high regularity, making it a very reliable attack indicator that cannot be concealed by an attacker. Test results show that our system can very accurately and quickly detect MITM attacks while requiring a simple learning approach.

==> note <==
gatttol referansi duzenlenecek authori yok cunku




eski tablolar

\begin{table*}[]
\vspace{0.5cm}

\footnotesize
\vspace{\baselineskip}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline

\textit{\textbf{Device Name}} & \textit{\textbf{Device Type}} & \textit{\textbf{Characteristic}}  & \textit{\textbf{Mean (sec) }} & \textit{\textbf{Variance (sec)}} & \textit{\textbf{Maximum (sec)}} & \textit{\textbf{Min (sec)}} & \textit{\textbf{FP}} & \textit{\textbf{FN}}  \\ \hline

LEDBLE             & Smart Bulb     & 0x000b                       & 0.03273  &  $  1.28261*10^{-13} $ & 0.032731   & 0.032729  & 0.00 & 0.00
\\ \hline
Mi Sensor                     & Temperature  Sensor   & 0x0043          &   0.03143   & $ 2.25594*10^{-5} $ &  0.050230 & 0.030229 & 0.06 & 0.00
\\ \hline
My Oximeter                   & Oximeter   & 0x0010                    &  0.05023   & $ 7.97839*10^{-11} $ & 0.050294  & 0.050229  & 0.00 & 0.00                                   
\\ \hline
Medical                       & Oximeter   & 0x0012                     &   0.01103    &  $ 3.14348*10^{-5} $ &  0.050326 & 0.010230  & 0.02 & 0.00                               
\\ \hline
MS1020                        & Smart Bracelet  & 0x001a                &  0.05073  &  $ 2.47513*10^{-5}  $ & 0.100231 & 0.050229 & 0.01 & 0.00
\\ \hline
iTag                        & Smart Tag       & 0x000b                &  0.18908   & $ 1.1834*10^{-2}  $ & 0.285228  & 0.048978   & 0.02 & 0.00                                   
\\ \hline
[TV] Samsung 7 Series         & Smart TV      & 0x002c                      & 0.07080  & $ 1.81988*10^{-3} $ &  0.243979   & 0.048518 & 0.11 & 0.16                                           
\\\hline
\end{tabular} 
\caption{Device List Write Operation Interval List (500 measurements)}
\label{fig:deviceintervallist}
\end{table*}


\begin{table*}[]
\vspace{0.5cm}

\footnotesize
\vspace{\baselineskip}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline

\textit{\textbf{Device Name}} & \textit{\textbf{Device Type}} & \textit{\textbf{Characteristic}}  & \textit{\textbf{Mean (sec) }} & \textit{\textbf{Variance (sec)}} & \textit{\textbf{Maximum (sec)}} & \textit{\textbf{Min (sec)}} & \textit{\textbf{FP}} & \textit{\textbf{FN}}  \\ \hline

LEDBLE            & Smart Bulb     & 0x0003   & 0.03023  &  $  9.72441*10^{-14} $ & 0.030230   & 0.030229  & &
\\ \hline
Mi Sensor         & Temperature  Sensor   & 0x0003          &   0.03023   & $ 6.08422*10^{-14} $ &  0.030230 & 0.030230  & &
\\ \hline
My Oximeter       & Oximeter   &                     &     & $  $ &   &  &  &                                 
\\ \hline
Medical           & Oximeter   & 0x0003                     &   0.01023    &  $ 7.46476*10^{-14} $ &  0.010231 & 0.010229     & &                         
\\ \hline
MS1020            & Smart Bracelet  & 0x0003                &  0.11938  &  $ 7.43592*10^{-3}  $ & 0.225229 & 0.048979  & &
\\ \hline
iTag              & Smart Tag       & 0x0003                &  0.23647   & $ 7.03120*10^{-3}  $ &  0.273978  & 0.048978     & &                            
\\ \hline
[TV] Samsung 7 Series         & Smart TV      & 0x0016                      & 0.05739  & $ 5.21485*10^{-4} $ &  0.146480    &  0.048464 &     &                                
\\\hline
\end{tabular} 
\caption{Device List Read Operation Interval List (500 measurements)}
\label{fig:deviceintervallist}
\end{table*}


\begin{figure}[!htb]
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev1.png}
  \caption{LEDBLE-7862E17D}\label{fig:dev1}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev3.png}
  \caption{My Oximeter}\label{fig:dev3}
\endminipage
\end{figure}

\begin{figure}[!htb]
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev6.png}
  \caption{iTag}\label{fig:dev6}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev7.png}
  \caption{[TV] Samsung 7 Series}\label{fig:dev7}
\endminipage
\end{figure}








COLUMN


\begin{figure}[!htb]
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev1.png}
  \caption{LEDBLE-7862E17D}\label{fig:dev1}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev2.png}
  \caption{LYWSD03MMC}\label{fig:dev2}
\endminipage
\end{figure}

\begin{figure}[!htb]
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev3.png}
  \caption{My Oximeter}\label{fig:dev3}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev4.png}
  \caption{Medical}\label{fig:dev4}
\endminipage
\end{figure}

\begin{figure}[!htb]
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev5.png}
  \caption{MS1020}\label{fig:dev5}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev6.png}
  \caption{iTag}\label{fig:dev6}
\endminipage
\end{figure}

\begin{figure}[!htb]
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev7.png}
  \caption{[TV] Samsung 7 Series}\label{fig:dev7}
\endminipage\hfill

\end{figure}















full devices


\begin{figure*}[!htb]

\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev1.png}
  \caption{LEDBLE}\label{fig:dev1}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev2.png}
  \caption{LYWSD03MMC}\label{fig:dev2}
\endminipage
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev3.png}
  \caption{My Oximeter}\label{fig:dev3}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev4.png}
  \caption{Medical}\label{fig:dev4}
\endminipage

\end{figure*}

\begin{figure*}[!htb]
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev5.png}
  \caption{MS1020}\label{fig:dev5}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev6.png}
  \caption{iTag}\label{fig:dev6}
\endminipage
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{dev-profiles/dev7.png}
  \caption{Samsung [TV]}\label{fig:dev7}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{}
\endminipage\hfill
\end{figure*}










TABLO KARAKTERISTIKLER OLMADAN


\begin{table*}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textit{\textbf{Device Name}}              & \textit{\textbf{Device Type}}   & \textit{\textbf{Operation}}  & \textit{\textbf{Mean (sec)}} & \textit{\textbf{Variance (sec)}} & \textit{\textbf{Maximum (sec)}} & \textit{\textbf{Min (sec)}} & \textit{\textbf{FP (\%)}} & \textit{\textbf{FN (\%)}} \\ \hline
\multirow{2}{*}{LEDBLE}                    & \multirow{2}{*}{Smart Bulb}         & \textbf{Read}                                 & 0.03023                      & $ 9.72441*10^{-14} $                            & 0.030230                        & 0.030229                    & 0.00                 & 0.00                 \\ \cline{3-9} 
                                           &                                     & \textbf{Write}                                 & 0.03273                     & $ 1.28261*10^{-13} $                            & 0.032731                        & 0.032729                    & 0.00                 & 0.00                 \\ \hline
\multirow{2}{*}{LYWSD03MMC}                 & \multirow{2}{*}{Termometer} & \textbf{Read}                                  & 0.03023                      & $ 6.08422*10^{-14} $                            & 0.030230                        & 0.030230                    & 0.00                 & 0.00                 \\ \cline{3-9} 
                                           &                                     & \textbf{Write}                                 & 0.03103                      & $ 1.53597*10^{-5} $                            & 0.050230                        & 0.030229                    & 4.00                 & 0.00                 \\ \hline
\multirow{2}{*}{My Oximeter}               & \multirow{2}{*}{Oximeter}           & \textbf{Read}                                  & 0.05008                      & $ 1.58237*10^{-7} $                            & 0.050230                        & 0.048979                    & 0.00                 & 0.00                 \\ \cline{3-9} 
                                           &                                     & \textbf{Write}                                 & 0.05023                      & $ 7.97839*10^{-11} $                            & 0.050294                        & 0.050229                    & 0.00                 & 0.00                 \\ \hline
\multirow{2}{*}{Medical}                   & \multirow{2}{*}{Oximeter}           & \textbf{Read}                                  & 0.01023                      & $ 7.46476*10^{-14} $                            & 0.010231                        & 0.010229                    & 0.00                 & 0.00                 \\ \cline{3-9} 
                                           &                                     & \textbf{Write}                                 & 0.01103                      & $ 3.14348*10^{-5} $                            & 0.050326                        & 0.010230                    & 2.00                 & 0.00                 \\ \hline
\multirow{2}{*}{MS1020}                    & \multirow{2}{*}{Smart Bracelet}     & \textbf{Read}                                 & 0.10998                      & $ 6.84789*10^{-3} $                            & 0.225229                        & 0.048979                    & 0.00                 & 0.00                 \\ \cline{3-9} 
                                           &                                     & \textbf{Write}                                & 0.05073                      & $ 2.47513*10^{-5} $                            & 0.100231                        & 0.050229                    & 1.00                 & 0.00                 \\ \hline
\multirow{2}{*}{iTag}                      & \multirow{2}{*}{Smart Tag}          & \textbf{Read}                                  & 0.23647                      & $ 7.03120*10^{-3} $                            & 0.273978                        & 0.048978                    & 0.00                 & 0.00                 \\ \cline{3-9} 
                                           &                                     & \textbf{Write}                                 & 0.18908                      & $ 1.1834*10^{-2} $                            & 0.285228                        & 0.048978                    & 2.00                 & 0.00                 \\ \hline
\multirow{2}{*}{ Samsung {[}TV{]}} & \multirow{2}{*}{Smart TV}           & \textbf{Read}                                 & 0.05739                      & $ 5.21485*10^{-4} $                            & 0.146480                        & 0.048464                    & 4.00                 & 16.00                 \\ \cline{3-9} 
                                           &                                     & \textbf{Write}                                 & 0.07080                      & $ 1.81988*10^{-3} $                            & 0.243979                        & 0.048518                    & 3.00                 & 16.00                 \\ \hline
\multicolumn{5}{l}{\textbf{}}                                                                                                                                                                                                                                                                               & \multicolumn{1}{l|}{}           & \textbf{Average}            & \textbf{1.14}        & \textbf{2.28}        \\ \cline{7-9} 

\end{tabular}
\caption{ATT Operation Interval List (250 legitimate 100 attack measurements)}
\label{fig:deviceintervallist}
\end{table*}





















WiSec 2021
ACM Conference on Security and Privacy in Wireless and Mobile Networks
June 28 – July 1 // Virtual, Abu Dhabi, UAE
22 days 22h 23m 55s
Deadline: 19 Mar 2021, 2:59:59 pm






==> notes <==

Sonuclar.
min false positive rate where true positive is 1
0.5828571428571429    -   divider 32.75

max true positive - false positive
0.7357142857142858 - 50.35

# mitm tek interfacele yapamiyoruz diyebilriiz.

# mitm detectionda profilleme ile ilgili problem var  var olan yontemlerin avantajlari common problem varsayilan.
# saldiri tool fingerprinting

2 asamali cozum
 - Advirtisement paketlerini takip etmek
        3 kanal bu ise ayrildigi icin takip devamli takip etmek mumkun
        - Eger baglantid evam ediyor mu, diye dogrulayip tekrar advertisemen goruyorsam kesin yakaliyorum. Bu durumda sniff etemeyi durdurmak gerekecek. Ya da server kadar, sniffer ihtiyac var. Veya wide-band sniffer'a ihtiyac var. 10bin USD-pahali. 
        - Alternatif olarak, cok adv+conn_req paketleri goruyorsam, direk yeni adv gordugumde saldiri alarmi verebilirim.
            Soru: Conn_req geldikten sonra bir cihaz neden baglanmiyabilir? 

            Cevap: takilabilir/bu mumkun degil. random mac adresi ile baglanti yapilmak istendiginde cihaza connection request gitmiyor. reddedecekse eger advertisei su sekilde gonderiyor.

            Linkte yazana gore connectable advertisement gonderiyorsa baglanmasi bekleniyor. https://devzone.nordicsemi.com/f/nordic-q-a/28000/can-a-ble-peripheral-conditionally-reject-connection-request-from-ble-central
            https://www.novelbits.io/bluetooth-low-energy-sniffer-tutorial-advertisements/
            ADV_IND'lere bakiyoruz diyecegiz.

            Soru 2: Bu durumda, server yeni adv'a ne zaman basliyor - MUHTEMELEN PROTOKOLDE TANIMLI: VEYA IMPLEMENTASYON DEPENDENT?
                            Soru-Soru2: Bir servera  conn-request gonderdin ve baglanmadin, pratikte 7 server ne yapiyor?

            Soru 3: Attack took, akilli modda, connection yaptiktan sonra adv'a ne zaman basliyor? Periodisite bozuluyor mu?
            Cevap 3: Attack toollar, periyodik olmayan intervaller gosteriyor. 0.5 saniyeyle 5 saniye arasinda intervaller gozlemledim. Duzgun bir dagilim yok. 3 toolu da test edip maximum gecikme olculebilir.
    
            Senaryo - Pair edemedi reddetti, kendisi advertisementa dondu. Saldirgan diye isaretledik. MITM deneyecek ama calismayacak Auth var mi yok mu bilirsek karar verebiliyoruz.
            
            Soru 4:  Bir cihaz baglanti saglandiktan sonra advertise yapmaya devam ediyor mu? Cihazdan cihaza degisiyor ancak test edilebilir bu. Fazladan baglantiya izin veriyor mu? BLE 4.0 cihazlar multiple connection kurdurtmuyor. 4.1den sonra Yeni cihazlar multiple master baglanmasina izin veriyor.Advertise yapabilir. Ama biz zaten eskilere bakiyoruz. Burada seti tanimlamak onemli gibi duruyor. Cok ihtimal var nasil cover edecegiz?

            30 saniye bekleyince cozuluyor.
            
            Cevap 4 : Blueshield genelde enable edilmedigini not etmis. Enable etmis olsa bile ayni mac adresine yonelik frekansi artacak. Preset valueiyla ya da flood yapiyor. adv frekansi artacak PCAP dosyasi var analizimiz dogru frekans 2 katina cikiyor. Yeni cihaz ekledik sisteme.

            Ayrica mac spoof edilmemis olabilir cihaz ismine bakilacak scan req response seklinde

            adv interval bakilir device name icin 
            sonra anomali        
        
 - Baslangic asamasi gorulmediyse o zaman zaman gecikmesi
        - Benzer yaklasim burada da kullanilabilir: 37 kanal dinlenip, replay girisimleri yakalanmaya calisabilir. Ancak bu fisible degil.
    
        - Alternatif olarak zaman gecikmesi gozlemlenebilir. 3 arac icin bulgular
        - Zaman gecikmesi --hareketli olarak olculurken-- RSSI nasil degisiyor? RSSI mesafeye gore oluyor.

MITM Detection Subsection

Recent Attack
     CTKD blurtooth, mitm yapilabilir oluyor.
     Firmxray mitm saldirilari yuzde 70 

mirage ile intervallere bak 3 profilleme ?
# LEDBLE ve  uzerinde meanleri cikararak                                                         
# ortalamalara bakarak kiyaslayacagiz

# 3. basamagin efektleri
# 1  3. traffic compromise
# 2  attack tool tespit
# 3 ele gecirilmis bir cihazi tespit etmek icin

# ilk baglantiyi gordum
    proxy connection var 
# ilk baglantiyi gormedigim baglanti
    proxy connection yok
# tablo 1 minimum meane degil
# attack privilege yukseltme
# process test tekrar edilecek

# 200 adet test
# mirage - ledble  114.96232988 ms diff mean mitm (0.03273) 16 ms 

kernel interval - ona en cihazin gecikmesi
-> minimum gecikme 20 dedik (haberimiz yok)
-> atak scheduling interval fonksiyonudur.

nice - process
4,5 ms 

timestamp 3 ms, mirage
->

# btlejuice - ledble  70.8753874 ms diff mean mitm (0.03273)
# gattacker - ledble  94.438698744 ms diff mean mitm (0.03273)

# mirage - my oximeter  65.35122396 ms diff mean mitm (0.5023)
# btlejuice - my oximeter  69.6177685 ms diff mean mitm (0.5023)
# gattacker - my oximeter  59.346610761 ms diff mean mitm (0.5023)


\\bin\\cmd\_btlejuice.js BLENO\_ADVERTISING\_INTERVAL
config.env BLENO\_ADVERTISING\_INTERVAL
mirage\\modules\\ble\_adv.py INTERVAL\_MIN, INTERVAL\_MAX

Minimum Deviation \\
BTLEJuice icin 16.250610 \\ % minplotter.py kodunda
Gattacker icin 17.49920  \\ % stats_ledble_gattacker.py kodunda
Mirage icin 32.497 \\ % stats_ledble_mirage.py kodunda

% https://mathcracker.com/normal-probability-grapher#results sitesinde yaptigim grafik 

mean=31.43021, standard dev =4.77360 olan cihaz icin grafik\\

We have the following graph to the corresponds to the specified event 
input step karismis




Results 
min false positive rate where true positive is 1 \\
0.5828571428571429    -   divider 32.75 \\

max true positive - false positive \\
0.7357142857142858 - 50.35 \\


konferanslar ve tarihleri

raid 2020
Blueshield
https://raid2020.org/call-for-papers/
Paper Submission Deadline:
March 24, 2020,


Usenix

BLESA
Winter Deadline
    Refereed paper submissions due: Thursday, February 4, 2021, 11:59 pm AoE
    Early reject notification: March 12, 202Vancouver, B.C., Canada
https://www.usenix.org/conference/usenixsecurity21/call-for-papers


# bunun vvakti gecti
mobisys
https://www.sigmobile.org/mobisys/2020/
# Important Dates
Abstract Registration:	January 8th, 2021 AoE
Paper Submission:	January 15th, 2021 AoE
Early Rejection Notification:	March 1st, 2021
Notification of Acceptance:	March 25, 2021



# tam anlamadim  tarihleri ama yetismeyecek sanirim ama devam
iotbds 2021
http://www.iotbds.org/
Position Papers /Regular Papers
Due to current exceptional circumstances, the deadlines below apply to both position papers and regular papers submitted after December 21st.
Paper Submission: January 19, 2021
Authors Notification: February 24, 2021
Camera Ready and Registration: March 9, 2021



https://www.ndss-symposium.org/
may 22 last submission - july 
accepted papers https://www.ndss-symposium.org/ndss2020/accepted-papers/


Mobicom
2021 march 19
https://www.sigmobile.org/mobicom/2021/cfp.html
# accepted papers 
https://sigmobile.org/mobicom/2020/accepted.php



CCS 2021
ACM Conference on Computer and Communications Security
November 14–19 // Seoul, South Korea
11 days 01h 20m 49s
Deadline: 21 Jan 2021, 2:59:59 pm

2020 sindeki  paper FirmRay: Detecting BLE Link Layer Vulnerabilities from Configurations in Bare-Metal Firmware


safe things 2021

https://www.ieee-security.org/TC/SP2021/SPW2021/safethings2021/
25 ocak
en uygunu bu gibi duruyor
bura gibi yaziyoruz.

problemlilerde arttir ve olcumleri ve histogram

==> notes-old <==

Sonuclar.
min false positive rate where true positive is 1
0.5828571428571429    -   divider 32.75

max true positive - false positive
0.7357142857142858 - 50.35

# mitm tek interfacele yapamiyoruz diyebilriiz.

# mitm detectionda profilleme ile ilgili problem var  var olan yontemlerin avantajlari common problem varsayilan.
# saldiri tool fingerprinting

2 asamali cozum
 - Advirtisement paketlerini takip etmek
        3 kanal bu ise ayrildigi icin takip devamli takip etmek mumkun
        - Eger baglantid evam ediyor mu, diye dogrulayip tekrar advertisemen goruyorsam kesin yakaliyorum. Bu durumda sniff etemeyi durdurmak gerekecek. Ya da server kadar, sniffer ihtiyac var. Veya wide-band sniffer'a ihtiyac var. 10bin USD-pahali. 
        - Alternatif olarak, cok adv+conn_req paketleri goruyorsam, direk yeni adv gordugumde saldiri alarmi verebilirim.
            Soru: Conn_req geldikten sonra bir cihaz neden baglanmiyabilir? 

            Cevap: takilabilir/bu mumkun degil. random mac adresi ile baglanti yapilmak istendiginde cihaza connection request gitmiyor. reddedecekse eger advertisei su sekilde gonderiyor.

            Linkte yazana gore connectable advertisement gonderiyorsa baglanmasi bekleniyor. https://devzone.nordicsemi.com/f/nordic-q-a/28000/can-a-ble-peripheral-conditionally-reject-connection-request-from-ble-central
            https://www.novelbits.io/bluetooth-low-energy-sniffer-tutorial-advertisements/
            ADV_IND'lere bakiyoruz diyecegiz.

            Soru 2: Bu durumda, server yeni adv'a ne zaman basliyor - MUHTEMELEN PROTOKOLDE TANIMLI: VEYA IMPLEMENTASYON DEPENDENT?
                            Soru-Soru2: Bir servera  conn-request gonderdin ve baglanmadin, pratikte 7 server ne yapiyor?

            Soru 3: Attack took, akilli modda, connection yaptiktan sonra adv'a ne zaman basliyor? Periodisite bozuluyor mu?
            Cevap 3: Attack toollar, periyodik olmayan intervaller gosteriyor. 0.5 saniyeyle 5 saniye arasinda intervaller gozlemledim. Duzgun bir dagilim yok. 3 toolu da test edip maximum gecikme olculebilir.
    
            Senaryo - Pair edemedi reddetti, kendisi advertisementa dondu. Saldirgan diye isaretledik. MITM deneyecek ama calismayacak Auth var mi yok mu bilirsek karar verebiliyoruz.
            
            Soru 4:  Bir cihaz baglanti saglandiktan sonra advertise yapmaya devam ediyor mu? Cihazdan cihaza degisiyor ancak test edilebilir bu. Fazladan baglantiya izin veriyor mu? BLE 4.0 cihazlar multiple connection kurdurtmuyor. 4.1den sonra Yeni cihazlar multiple master baglanmasina izin veriyor.Advertise yapabilir. Ama biz zaten eskilere bakiyoruz. Burada seti tanimlamak onemli gibi duruyor. Cok ihtimal var nasil cover edecegiz?

            30 saniye bekleyince cozuluyor.
            
            Cevap 4 : Blueshield genelde enable edilmedigini not etmis. Enable etmis olsa bile ayni mac adresine yonelik frekansi artacak. Preset valueiyla ya da flood yapiyor. adv frekansi artacak PCAP dosyasi var analizimiz dogru frekans 2 katina cikiyor. Yeni cihaz ekledik sisteme.

            Ayrica mac spoof edilmemis olabilir cihaz ismine bakilacak scan req response seklinde

            adv interval bakilir device name icin 
            sonra anomali        
        
 - Baslangic asamasi gorulmediyse o zaman zaman gecikmesi
        - Benzer yaklasim burada da kullanilabilir: 37 kanal dinlenip, replay girisimleri yakalanmaya calisabilir. Ancak bu fisible degil.
    
        - Alternatif olarak zaman gecikmesi gozlemlenebilir. 3 arac icin bulgular
        - Zaman gecikmesi --hareketli olarak olculurken-- RSSI nasil degisiyor? RSSI mesafeye gore oluyor.

MITM Detection Subsection

Recent Attack
     CTKD blurtooth, mitm yapilabilir oluyor.
     Firmxray mitm saldirilari yuzde 70 

mirage ile intervallere bak 3 profilleme ?
# LEDBLE ve  uzerinde meanleri cikararak                                                         
# ortalamalara bakarak kiyaslayacagiz

# 3. basamagin efektleri
# 1  3. traffic compromise
# 2  attack tool tespit
# 3 ele gecirilmis bir cihazi tespit etmek icin

# ilk baglantiyi gordum
    proxy connection var 
# ilk baglantiyi gormedigim baglanti
    proxy connection yok
# tablo 1 minimum meane degil
# attack privilege yukseltme
# process test tekrar edilecek

# 200 adet test
# mirage - ledble  114.96232988 ms diff mean mitm (0.03273) 16 ms 

kernel interval - ona en cihazin gecikmesi
-> minimum gecikme 20 dedik (haberimiz yok)
-> atak scheduling interval fonksiyonudur.

nice - process
4,5 ms 

timestamp 3 ms, mirage
->

# btlejuice - ledble  70.8753874 ms diff mean mitm (0.03273)
# gattacker - ledble  94.438698744 ms diff mean mitm (0.03273)

# mirage - my oximeter  65.35122396 ms diff mean mitm (0.5023)
# btlejuice - my oximeter  69.6177685 ms diff mean mitm (0.5023)
# gattacker - my oximeter  59.346610761 ms diff mean mitm (0.5023)


\\bin\\cmd\_btlejuice.js BLENO\_ADVERTISING\_INTERVAL
config.env BLENO\_ADVERTISING\_INTERVAL
mirage\\modules\\ble\_adv.py INTERVAL\_MIN, INTERVAL\_MAX

Minimum Deviation \\
BTLEJuice icin 16.250610 \\ % minplotter.py kodunda
Gattacker icin 17.49920  \\ % stats_ledble_gattacker.py kodunda
Mirage icin 32.497 \\ % stats_ledble_mirage.py kodunda

% https://mathcracker.com/normal-probability-grapher#results sitesinde yaptigim grafik 

mean=31.43021, standard dev =4.77360 olan cihaz icin grafik\\

We have the following graph to the corresponds to the specified event 
input step karismis




Results 
min false positive rate where true positive is 1 \\
0.5828571428571429    -   divider 32.75 \\

max true positive - false positive \\
0.7357142857142858 - 50.35 \\


konferanslar ve tarihleri

raid 2020
Blueshield
https://raid2020.org/call-for-papers/
Paper Submission Deadline:
March 24, 2020,


Usenix

BLESA
Winter Deadline
    Refereed paper submissions due: Thursday, February 4, 2021, 11:59 pm AoE
    Early reject notification: March 12, 202Vancouver, B.C., Canada
https://www.usenix.org/conference/usenixsecurity21/call-for-papers


# bunun vvakti gecti
mobisys
https://www.sigmobile.org/mobisys/2020/
# Important Dates
Abstract Registration:	January 8th, 2021 AoE
Paper Submission:	January 15th, 2021 AoE
Early Rejection Notification:	March 1st, 2021
Notification of Acceptance:	March 25, 2021



# tam anlamadim  tarihleri ama yetismeyecek sanirim ama devam
iotbds 2021
http://www.iotbds.org/
Position Papers /Regular Papers
Due to current exceptional circumstances, the deadlines below apply to both position papers and regular papers submitted after December 21st.
Paper Submission: January 19, 2021
Authors Notification: February 24, 2021
Camera Ready and Registration: March 9, 2021



https://www.ndss-symposium.org/
may 22 last submission - july 
accepted papers https://www.ndss-symposium.org/ndss2020/accepted-papers/

# ndss' pasif aktif birleştirme.



Mobicom
2021 march 19
https://www.sigmobile.org/mobicom/2021/cfp.html
# accepted papers 
https://sigmobile.org/mobicom/2020/accepted.php



CCS 2021
ACM Conference on Computer and Communications Security
November 14–19 // Seoul, South Korea
11 days 01h 20m 49s
Deadline: 21 Jan 2021, 2:59:59 pm

2020 sindeki  paper FirmRay: Detecting BLE Link Layer Vulnerabilities from Configurations in Bare-Metal Firmware


safe things 2021

https://www.ieee-security.org/TC/SP2021/SPW2021/safethings2021/
25 ocak
en uygunu bu gibi duruyor
bura gibi yaziyoruz.

problemlilerde arttir ve olcumleri ve histogram

==> referanslar-old <==
@inproceedings{wang2020bluedoor,
  title={BlueDoor: breaking the secure information flow via BLE vulnerability},
  author={Wang, Jiliang and Hu, Feng and Zhou, Ye and Liu, Yunhao and Zhang, Hanyi and Liu, Zhe},
  booktitle={Proceedings of the 18th International Conference on Mobile Systems, Applications, and Services},
  pages={286--298},
  year={2020}
}
@inproceedings {255346,
author = {Yue Zhang and Jian Weng and Rajib Dey and Yier Jin and Zhiqiang Lin and Xinwen Fu},
title = {Breaking Secure Pairing of Bluetooth Low Energy Using Downgrade Attacks},
booktitle = {29th {USENIX} Security Symposium ({USENIX} Security 20)},
year = {2020},
isbn = {978-1-939133-17-5},
pages = {37--54},
url = {https://www.usenix.org/conference/usenixsecurity20/presentation/zhang-yue},
publisher = {{USENIX} Association},
month = aug,
}

@inproceedings{fawaz2016protecting,
  title={Protecting privacy of $\{$BLE$\}$ device users},
  author={Fawaz, Kassem and Kim, Kyu-Han and Shin, Kang G},
  booktitle={25th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 16)},
  pages={1205--1221},
  year={2016}
}

@inproceedings{celosia2019fingerprinting,
  title={Fingerprinting Bluetooth-Low-Energy Devices Based on the Generic Attribute Profile},
  author={Celosia, Guillaume and Cunche, Mathieu},
  booktitle={Proceedings of the 2nd International ACM Workshop on Security and Privacy for the Internet-of-Things},
  pages={24--31},
  year={2019}
}


@inproceedings{siby2017iotscanner,
  title={Iotscanner: Detecting privacy threats in iot neighborhoods},
  author={Siby, Sandra and Maiti, Rajib Ranjan and Tippenhauer, Nils Ole},
  booktitle={Proceedings of the 3rd ACM International Workshop on IoT Privacy, Trust, and Security},
  pages={23--30},
  year={2017}
}

@article{watkins2016tattle,
  title={Tattle Tale Security: An Intrusion Detection System for Medical Body Area Networks (MBAN)},
  author={Watkins, Lanier and Aggarwal, Shreya and Akeredolu, Omotola and Robinson, William H and Rubin, Aviel},
  year={2016}
}

@article{yaseen2019marc,
  title={MARC: A Novel Framework for Detecting MITM Attacks in eHealthcare BLE Systems},
  author={Yaseen, Muhammad and Iqbal, Waseem and Rashid, Imran and Abbas, Haider and Mohsin, Mujahid and Saleem, Kashif and Bangash, Yawar Abbas},
  journal={Journal of Medical Systems},
  volume={43},
  number={11},
  pages={324},
  year={2019},
  publisher={Springer}
}

@inproceedings{jeannotte2019artorias,
  title={Artorias: IoT Security Testing Framework},
  author={Jeannotte, Bryer and Tekeoglu, Ali},
  booktitle={2019 26th International Conference on Telecommunications (ICT)},
  pages={233--237},
  year={2019},
  organization={IEEE}
}

@inproceedings{das2016uncovering,
  title={Uncovering privacy leakage in ble network traffic of wearable fitness trackers},
  author={Das, Aveek K and Pathak, Parth H and Chuah, Chen-Nee and Mohapatra, Prasant},
  booktitle={Proceedings of the 17th International Workshop on Mobile Computing Systems and Applications},
  pages={99--104},
  year={2016}
}



@article{acar2018peek,
  title={Peek-a-Boo: I see your smart home activities, even encrypted!},
  author={Acar, Abbas and Fereidooni, Hossein and Abera, Tigist and Sikder, Amit Kumar and Miettinen, Markus and Aksu, Hidayet and Conti, Mauro and Sadeghi, Ahmad-Reza and Uluagac, A Selcuk},
  journal={arXiv preprint arXiv:1808.02741},
  year={2018}
}

@article{hafeez2020iot,
  title={IoT-KEEPER: Detecting malicious IoT network activity using online traffic analysis at the edge},
  author={Hafeez, Ibbad and Antikainen, Markku and Ding, Aaron Yi and Tarkoma, Sasu},
  journal={IEEE Transactions on Network and Service Management},
  volume={17},
  number={1},
  pages={45--59},
  year={2020},
  publisher={IEEE}
}

@inproceedings{albazrqaoe2016practical,
  title={Practical bluetooth traffic sniffing: Systems and privacy implications},
  author={Albazrqaoe, Wahhab and Huang, Jun and Xing, Guoliang},
  booktitle={Proceedings of the 14th Annual International Conference on Mobile Systems, Applications, and Services},
  pages={333--345},
  year={2016}
}

@inproceedings{sarkar2019robust,
  title={A Robust Algorithm for Sniffing BLE Long-Lived Connections in Real-time},
  author={Sarkar, Sopan and Liu, Jianqing and Jovanov, Emil},
  booktitle={2019 IEEE Global Communications Conference (GLOBECOM)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@article{lounis2020attacks,
  title={Attacks and Defenses in Short-Range Wireless Technologies for IoT},
  author={Lounis, Karim and Zulkernine, Mohammad},
  journal={IEEE Access},
  volume={8},
  pages={88892--88932},
  year={2020},
  publisher={IEEE}
}

@article{sun2018man,
  title={Man-in-the-middle attacks on Secure Simple Pairing in Bluetooth standard V5. 0 and its countermeasure},
  author={Sun, Da-Zhi and Mu, Yi and Susilo, Willy},
  journal={Personal and Ubiquitous Computing},
  volume={22},
  number={1},
  pages={55--67},
  year={2018},
  publisher={Springer}
}

@article{wublueshield,
  title={BlueShield: Detecting Spoofing Attacks in Bluetooth Low Energy Networks},
  author={Wu, Jianliang and Nan, Yuhong and Kumar, Vireshwar and Payer, Mathias and Xu, Dongyan}
}

@misc{bluetoothsig,
  author = {{Bluetooth SIG}},
  title = {Bluetooth Market Update},
  howpublished = {https://www.bluetooth.com/bluetooth-resources/2020-bmu/},
  note = {Accessed Date: 2020-07-24}
}

@misc{blesecureconnections,
  author = {{Bluetooth SIG}},
  title = {Core Specifications 5.2},
  howpublished = {https://www.bluetooth.com/specifications/bluetooth-core-specification/},
  note = {Page: 1641, Accessed Date: 2020-08-05}
}

@misc{gattcharacteristics,
  author ={{Bluetooth SIG}},
  title = {GATT Characteristics},
  howpublished = {https://www.bluetooth.com/specifications/gatt/characteristics/},
  note = {Accessed Date: 2020-08-05}
}

@inproceedings{8728448,  author={S. {Pallavi} and V. A. {Narayanan}},  booktitle={2019 5th International Conference on Advanced Computing   Communication Systems (ICACCS)},   title={An Overview of Practical Attacks on BLE Based IOT Devices and Their Security},   year={2019},  volume={},  number={},  pages={694-698},}

@article{iotattacks,
author = {Hezam, Akram and Konstantas, Dimitri and Mahyoub, Mohammed},
year = {2018},
month = {04},
pages = {},
title = {A Comprehensive IoT Attacks Survey based on a Building-blocked Reference Mode},
volume = {Vol. 9},
journal = {International Journal of Advanced Computer Science and Applications},
doi = {10.14569/IJACSA.2018.090349}
}

@article{Lonzetta2018SecurityVI,
  title={Security Vulnerabilities in Bluetooth Technology as Used in IoT},
  author={Angela M. Lonzetta and Peter Cope and Joseph Campbell and Bassam Jamil Mohd and Thaier Hayajneh},
  journal={J. Sensor and Actuator Networks},
  year={2018},
  volume={7},
  pages={28}
}

@inproceedings{garbelini2020sweyntooth,
  title={SweynTooth: Unleashing Mayhem over Bluetooth Low Energy},
  author={Garbelini, Matheus E and Wang, Chundong and Chattopadhyay, Sudipta and Sumei, Sun and Kurniawan, Ernest},
  booktitle={2020 $\{$USENIX$\}$ Annual Technical Conference ($\{$USENIX$\}$$\{$ATC$\}$ 20)},
  pages={911--925},
  year={2020}
}

@inproceedings{ryan2013bluetooth,
  title={Bluetooth: With low energy comes low security},
  author={Ryan, Mike},
  booktitle={7th $\{$USENIX$\}$ Workshop on Offensive Technologies ($\{$WOOT$\}$ 13)},
  year={2013}
}

@article{energy2019bluetooth,
  title={Bluetooth Low Energy (BLE) Security and Privacy},
  author={Energy, Bluetooth Low},
  year={2019}
}
@misc{crackle,
  author = {{mikeryan}},
  title = {Crackle},
  howpublished = {https://github.com/mikeryan/crackle},
  note = {Accessed Date: 2020-08-05}
}

@misc{gattacker,
  author = {{Securing}},
  title = {Gattacker},
  howpublished = {https://github.com/securing/gattacker},
  note = {Accessed Date: 2020-08-05}
}

@misc{gatttool,
  author = {{Securing}},
  title = {Gatttool},
  howpublished = {http://manpages.ubuntu.com/manpages/cosmic/man1\\/gatttool.1.html},
  note = {Accessed Date: 2020-08-05}
}

@misc{bluepy,
  author = {{IanHarvey}},
  title = {bluepy},
  howpublished = {https://github.com/IanHarvey/bluepy},
  note = {Accessed Date: 2020-08-05}
}

@misc{mirage,
  author = {{RCayre}},
  title = {mirage},
  howpublished = {https://github.com/RCayre/mirage},
  note = {Accessed Date: 2020-08-05}
}



@misc{btlejuice,
  author = {DigitalSecurity},
  title = {btlejuice},
  howpublished = {https://github.com/DigitalSecurity/btlejuice},
  note = {Accessed Date: 2020-08-05}
}

@misc{connecteddevices,
  author = {{Bluetooth SIG}},
  title = {Connected Devices},
  howpublished = {https://www.bluetooth.com/learn-about-bluetooth/markets/connected-device/},
  note = {Accessed Date: 2020-09-21}
}



@misc{blurtooth,
  author = {{National Vulnerability Database}},
  title = {{CVE-2020-15802}},
  howpublished = {https://cve.mitre.org/cgi-bin/cvename.cgi?name=CVE-2020-15802},
  note = {Accessed Date: 2020-09-14}
}

@misc{bluetoothspec,
  author = {{Bluetooth SIG}},
  title = {Core Specifications 5.2},
  howpublished = {https://www.bluetooth.com/specifications/bluetooth-core-specification/},
  note = {Accessed Date: 2020-08-05}
}

@misc{blesecurity,
  author = {{NCC Group}},
  title = {Bluetooth 5 Hacking},
  howpublished = {https://hardwear.io/webinar/hwio\_bluetooth\_webinar.pdf},
  note = {Page: 10,Accessed Date: 2020-08-05}
}

@misc{assigned,
  author = {{Bluetooth SIG}},
  title = {Assigned Numbers},
  howpublished = {https://www.bluetooth.com/specifications/assigned-numbers},
  note = {Accessed Date: 2021-01-01}
}

@misc{bluetoothaddresses,
  author = {novelbits},
  title = {Bluetooth Addresses and Privacy in Bluetooth Low Energy},
  howpublished = {https://www.novelbits.io/bluetooth-address-privacy-ble/},
  note = {Accessed Date: 2020-08-05}
}
@misc{bluetoothclocks,
  author = {Elvis Pfützenreuter},
  title = {Bluetooth: clocks and CSP},
  howpublished = {https://epxx.co/artigos/bluetooth\_csp\_en.html},
  note = {Accessed Date: 2020-08-05}
}

@article{martin2019handoff,
  title={Handoff all your privacy--a review of apple’s bluetooth low energy continuity protocol},
  author={Martin, Jeremy and Alpuche, Douglas and Bodeman, Kristina and Brown, Lamont and Fenske, Ellis and Foppe, Lucas and Mayberry, Travis and Rye, Erik and Sipes, Brandon and Teplov, Sam},
  journal={Proceedings on Privacy Enhancing Technologies},
  volume={2019},
  number={4},
  pages={34--53},
  year={2019},
  publisher={Sciendo}
}

@inproceedings{kang2015review,
  title={A review of security protocols in mHealth wireless body area networks (WBAN)},
  author={Kang, James and Adibi, Sasan},
  booktitle={International Conference on Future Network Systems and Security},
  pages={61--83},
  year={2015},
  organization={Springer}
}

@article{alfian2018personalized,
  title={A personalized healthcare monitoring system for diabetic patients by utilizing BLE-based sensors and real-time data processing},
  author={Alfian, Ganjar and Syafrudin, Muhammad and Ijaz, Muhammad Fazal and Syaekhoni, M Alex and Fitriyani, Norma Latif and Rhee, Jongtae},
  journal={Sensors},
  volume={18},
  number={7},
  pages={2183},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{newaz2020survey,
  title={A Survey on Security and Privacy Issues in Modern Healthcare Systems: Attacks and Defenses},
  author={Newaz, AKM and Sikder, Amit Kumar and Rahman, Mohammad Ashiqur and Uluagac, A Selcuk},
  journal={arXiv preprint arXiv:2005.07359},
  year={2020}
}

@article{yang2020beyond,
  title={Beyond beaconing: Emerging applications and challenges of BLE},
  author={Yang, Jian and Poellabauer, Christian and Mitra, Pramita and Neubecker, Cynthia},
  journal={Ad Hoc Networks},
  volume={97},
  pages={102015},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{wu2020blesa,
  title={$\{$BLESA$\}$: Spoofing Attacks against Reconnections in Bluetooth Low Energy},
  author={Wu, Jianliang and Nan, Yuhong and Kumar, Vireshwar and Tian, Dave Jing and Bianchi, Antonio and Payer, Mathias and Xu, Dongyan},
  booktitle={14th $\{$USENIX$\}$ Workshop on Offensive Technologies ($\{$WOOT$\}$ 20)},
  year={2020}
}

@inproceedings{lahmadi2020mitm,
  title={MitM Attack Detection in BLE Networks using Reconstruction and Classification Machine Learning Techniques},
  author={Lahmadi, Abdelkader and Duque, Alexis and Heraief, Nathan and Francq, Julien},
  booktitle={MLCS 2020-2nd Workshop on Machine Learning for Cybersecurity},
  year={2020}
}

@inproceedings{galtier2020psd,
  title={A PSD-based fingerprinting approach to detect IoT device spoofing},
  author={Galtier, Florent and Cayre, Romain and Auriol, Guillaume and Ka{\^a}niche, Mohamed and Nicomette, Vincent},
  booktitle={25th IEEE Pacific Rim International Symposium on Dependable Computing (PRDC 2020)}
}

@inproceedings{wen2020firmxray,
  title={FirmXRay: Detecting Bluetooth Link Layer Vulnerabilities From Bare-Metal Firmware},
  author={Wen, Haohuang and Lin, Zhiqiang and Zhang, Yinqian},
  booktitle={Proceedings of the 2020 ACM SIGSAC Conference on Computer and Communications Security},
  pages={167--180},
  year={2020}
}

@article{kang2018trusted,
  title={Trusted Time-Based Verification Model for Automatic Man-in-the-Middle Attack Detection in Cybersecurity},
  author={Kang, James Jin and Fahd, Kiran and Venkatraman, Sitalakshmi},
  journal={Cryptography},
  volume={2},
  number={4},
  pages={38},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}


@inproceedings{vallivaara2014detecting,
  title={Detecting man-in-the-middle attacks on non-mobile systems},
  author={Vallivaara, Visa Antero and Sailio, Mirko and Halunen, Kimmo},
  booktitle={Proceedings of the 4th ACM conference on Data and application security and privacy},
  pages={131--134},
  year={2014}
}


